Tree pyramidal adaptive importance sampling

This paper introduces Tree-Pyramidal Adaptive Importance Sampling (TP-AIS), a novel iterated sampling method that outperforms state-of-the-art approaches like deterministic mixture population Monte Carlo (DM-PMC), mixture population Monte Carlo (M-PMC) and layered adaptive importance sampling (LAIS). TP-AIS iteratively builds a proposal distribution parameterized by a tree pyramid, where each tree leaf spans a subspace that represents its importance density. After each new sample operation, a set of tree leaves are subdivided for improving the approximation of the proposal distribution to the target density. Unlike the rest of the methods in the literature, TP-AIS is parameter free and requires no tuning to achieve its best performance. We evaluate TP-AIS with different complexity randomized target probability density functions (PDF) and also analyze its application to different dimensions. The results are compared to state-of-the-art iterative importance sampling approaches and other baseline MCMC approaches using Normalized Effective Sample Size (N-ESS), Jensen-Shannon Divergence, and time complexity.

==> appendices/applications.tex <==
\subsection{Object pose inference from depth images}

\subsection{Macro-molecular ligand-receptor docking}
Protein–protein interactions are involved in virtually all cellular processes, such as protein expression regulation, cell-cycle control or immune response, among many others (Eisenberg et al., 2000). Characterizing such interactions at atomic level is of paramount importance to better understand pathological conditions at molecular level.
\begin{itemize}
    \item Metrics: minimum energy, gibbs free energy
    \item Sota techniques: GSO sampling. PSO. 
    \item Score functions: Anisotropic Network Model allows certain flexibility in ligand and receptor. Adds about 20 dimensions to the problem. Force-field approaches. Free-energy computations.
    \item Interesting problem ADN - enzyme
\end{itemize}


==> appendices/evidence_approx.tex <==
The Tree Pyramid sampling approach partitions the space in hierarchical non-uniform convex hyper-volumes. This lets us compute the evidence by summation of each sample probability mass. First, we approximate the probability density inside each partition hyper-volume to be uniform, the evidence of the sampled posterior density function is thus approximated by:

$$ Z = \sum_{i=0}^N P(c_i|D)r_i^k,$$

where each discrete piece of evidence $Z_i$ is obtained by computing the probability mass contained in each hyper-volume using the sample radius $r_i$ and its likelihood value $P(c_i | D)$. Figure~\ref{fig:evidence_approximation} shows several examples of the evidence computed on a 1-D example with different posterior distributions and number of samples. This approximation relaxes the intractability problem of evidence computation for Bayesian inference applications and allows the computation of normalized probabilities.

\begin{figure}
    \centering
    \includegraphics[width=0.32\textwidth]{figures/evidence_approx_1.png}
    \includegraphics[width=0.32\textwidth]{figures/evidence_approx_2.png}
    \includegraphics[width=0.32\textwidth]{figures/evidence_approx_3.png}
    \caption{Evidence approximation on three different PDFs. The sampling space is bounded to [-1,1]. Left: A 1-D normal distribution with $\mu=0$ $\sigma=0.1$ approximated by 20 samples. Middle: A 1-D gaussian mixture model with $\mu=[0.4 -0.2]$ $\sigma=[0.01, 0.3]$ approximated by 100 samples. Right: A 1-D gaussian mixture model with $\mu=[0.4 -0.2]$ $\sigma=[0.01, 0.3]$ approximated by 100 samples.}
    \label{fig:evidence_approximation}
\end{figure}


==> appendices/pdf_approximation.tex <==
\subsection{PDF Approximation}
The result of a sampling algorithm is a set of samples drawn from the target PDF, a byproduct of AIS methods is the adapted proposal distribution. We evaluate how close to the true distribution the adapted proposal is, for MCMC algorithms we use a KDE approximation from the samples. For the continuous PDF fitting, two methods are used: Kernel Density Estimation and Nearest Neighbor Approximation. Figure~\ref{fig:PDF_approximation} shows an example of the two approximation methods on a bi-variate Gaussian mixture model distribution.

\subsubsection*{Kernel Density Estimation}
KDE is a well known method used to estimate an unknown PDF from its drawn samples \cite{Epanechnikov69}. Consider $\mathcal{X} = {x_0, \dots ,x_n }$ a set of samples drawn from an unknown PDF $P$, its Kernel Density Estimator $\hat{P}$ is
    $$\hat{P}(x) = \frac{1}{nh} \sum^{n-1}_{i=0} K\Big( \frac{x - x_i}{h} \Big),$$
where $K$ is a kernel function and $h$ is a smoothing parameter a.k.a. \textit{bandwidth}. For discussion about kernel and bandwidth selection criteria we refer the reader to \cite{jones96}. In this paper, we have used a Gaussian kernel function and manually tuned $h$ to fit the ground truth distribution. All the sampling methods compared in this paper use the same KDE kernel and bandwidth to obtain the sample-based PDF approximation.

\subsubsection*{Nearest Neighbor Approximation}
\todo[inline]{Explain how to normalize this approximation such that it integrates to 1 or why we can use it as is without needing to normalize.}
Unfortunately, the computational cost of computing the esimated density using a KDE estimator is $\mathcal{O}(N)$. In the evaluation process we consider both small and big sample sets, especially for the performance evaluation in higher dimensions. As an alternative to KDE we use a computationally tractable approximation function such as the nearest neighbor approximation with $\mathcal{O}(log(N))$ cost defined by:
$\hat{P}(x) = P(\mathcal{X}[argmin_i(||x-x_i||)])$.

\begin{figure}
    \centering
    \includegraphics[width=0.99\textwidth]{figures/pdf_approximation.png}
    \caption{Example of the PDFs approximation methods used for the experimental comparison with their corresponding similarity metrics. Right: Ground truth distribution, a Bi-variate Gaussian Mixture Model. Middle: Samples (obtained with our TP method) and its Kernel Density Estimate approximation with bandwidth = 0.02. Left: Nearest neighbor approximation.}
    \label{fig:PDF_approximation}
\end{figure}


==> appendices/sampling_methods.tex <==
\todo{Comment on general importance sampling and the relation of the importance weight to the evaluated sampling methods.}

\todo{Elaborate on the reasons to select the different sampling methods by commenting on their strengths and weaknesses.}

\subsubsection{Rejection Sampling}

\subsubsection{Uniform Importance Sampling}
- Simulated annealing

\subsubsection{Markov Chain Monte Carlo}
\paragraph{Metropolis-Hastings}

\paragraph{Hybrid Monte Carlo}

\subsubsection{Nested Sampling}
\todo{Comment on the nested sampling approach, its variations and the reason to use Multi-Nested Sampling.}

\section*{On sampling methods, thoughts and discussion}
The process of sampling consists on obtaining a subset of elements that are representative of a broader set. For the subset to be representative, it has to preserve the statistical properties of the super-set that it is representing. For example, imagine a city with a population of 10000 people and we're interested in their age (sample space). In the discrete case, simply sampling at random from the population is a good strategy to generate a subset that is representative. However, sometimes super-sets are continuous (have infinite elements) and are described by a probability density function (PDF). Generating samples from a continuous PDF is solved for Normal distributions using the Box-Mueller transform, the inverse distribution function or less efficiently using the central limit theorem. However if the PDF is complex, non-parametric or simply unknown we need other approaches to generate samples from it. In these cases is where other sampling techniques such as Importance Sampling, Simulated annealing, MCMC and so on become useful. Later, the samples can be used to build an approximation of the continuous PDF (e.g. using Kernel Density Estimation) that can be used to make inference about modes, mean, entropy, intervals etc.

